Angular dependent measurement of electron-ion recombination in liquid argon for ionization calorimetry in the ICARUS liquid argon time projection chamber

This paper reports on a measurement of electron-ion recombination in liquid argon in the ICARUS liquid argon time projection chamber (LArTPC). A clear dependence of recombination on the angle of the ionizing particle track relative to the drift electric field is observed. An ellipsoid modified box (EMB) model of recombination describes the data across all measured angles. These measurements are used for the calorimetric energy scale calibration of the ICARUS TPC, which is also presented. The impact of the EMB model is studied on calorimetric particle identification, as well as muon and proton energy measurements. Accounting for the angular dependence in EMB recombination improves the accuracy and precision of these measurements.

==> sections/Gain.tex <==
% Charge measurements, in terms of $dQ/dx$, are turned into $dE/dx$ measurements for application in particle identification and calorimetric energy reconstruction. This is done by multiplying the detected charge, measured in ADC, by the electronics gain, measured in $\# e^- / \mathrm{ADC}$. Then, a correction is applied to account for the amount of ionization electrons that re-combined with argon ions at the point of ionization. Recombination measurements have been performed in liquid argon at the ICARUS drift field \cite{NEUTRecomb, ICARUSrecomb}. Test bench measurements of the ICARUS electronics gain have also been performed CITE XXX. 

% These external measurements serve as a starting point. For the result presented here though, we have performed in-situ measurements of both the collection plane gain and recombination to determine the energy scale calibration. Presicely calibrating the induction plane gain is left to future work. The effective gain on the ICARUS collection planes departs from the test bench gain due to the effect of the induction wire plane in-transparency shadowing and uncertain amount of charge from the collection plane (see section \ref{sec:q=effect}). In addition, in ICARUS we observe an angular dependence in ionization recombination at large $dE/dx$ not conclusively demonstrated by any prior recombination measurement in LAr. We have found in ICARUS that accounting for the angular dependence in recombination is necessary to properly calibrate energy measurements (for use, e.g., in particle identification). The recombination measurement here is the first that is applicable for use in angular dependent recombination corrections in liquid argon.

% We use two ``standard-candles" in the energy scale calibration: stopping muons and protons. In both cases, at each hit along the track the expected $dE/dx$ can be inferred from the residual range in the track after that hit, as well as other relevant kinematic quantities. The energy loss scale for muon and proton particle tracks is discussed in section \ref{sec:energyscale}. By measuring the $dQ/dx$ (in ADC) along muon and proton tracks, the gain and recombination can be measured. We include hits from muons near the minimum-ionizing region, to provide information on low-ionization depositions, and hits from protons up to its endpoint, to provide information on high-ionization depositions. We do this fit in a combined way, including all muon and proton $dQ/dx$ measurements to extract values of the gain and (angular dependent) recombination in a single measurement. The fit procedure and its results are discussed in section \ref{sec:energy_fit}.

% Muons are identified from cathode-crossing cosmic muon tracks that stop inside the detector. Protons are identified from neutrino interactions. The procedure to select for these to populations is detailed in section \ref{sec:gain_selection}. 
